Kunlun: Establishing Scaling Laws for Massive-Scale Recommendation Systems through Unified Architecture Design

Deriving predictable scaling laws that govern the relationship between model performance and computational investment is crucial for designing and allocating resources in massive-scale recommendation systems. While such laws are established for large language models, they remain challenging for recommendation systems, especially those processing both user history and context features. We identify poor scaling efficiency as the main barrier to predictable power-law scaling, stemming from inefficient modules with low Model FLOPs Utilization (MFU) and suboptimal resource allocation. We introduce Kunlun, a scalable architecture that systematically improves model efficiency and resource allocation. Our low-level optimizations include Generalized Dot-Product Attention (GDPA), Hierarchical Seed Pooling (HSP), and Sliding Window Attention. Our high-level innovations feature Computation Skip (CompSkip) and Event-level Personalization. These advances increase MFU from 17% to 37% on NVIDIA B200 GPUs and double scaling efficiency over state-of-the-art methods. Kunlun is now deployed in major Meta Ads models, delivering significant production impact.

==> sections/0_abstract_v3.tex <==
\begin{abstract}
% \renewcommand{\thefootnote}{\fnsymbol{footnote}}
% \footnotetext{$^*$Equal contribution, $^\dagger$Corresponding author}
% \renewcommand{\thefootnote}{\arabic{footnote}}
% % Deriving predictable scaling laws that govern the relationship between model performance and computational investment is crucial for guiding system design and resource allocation in massive-scale recommendation systems. While such laws have been well-established for large language models, they remain an open challenge for recommendation systems, particularly for systems that jointly process rich user history (sequential features) and non-sequential context features. We identify poor \emph{scaling efficiency} as the primary barrier that prevents these systems from achieving predictable power-law scaling behaviors. Our analysis reveals that these bottlenecks arise from two main aspects: (1) \emph{inefficient modules} where models cannot fully utilize GPU computational resources, as measured by low Model FLOPs Utilization (MFU), due to heterogeneous feature spaces and small embedding dimensions, and (2) \emph{inefficient computation resource allocation} where resources are poorly distributed across model components. We propose \algname, a scalable architecture design that addresses these bottlenecks through systematic model-efficiency codesign. Our \emph{low-level} optimizations include Generalized Dot-Product Attention (GDPA) for efficient personalized sequence transformation, Hierarchical Seed Pooling (HSP) for effective sequence summarization, and Sliding Window Attention for linear-complexity sequence modeling, which address inefficient modules. Our \emph{high-level} innovations feature Computation Skip (CompSkip) for layer-wise component selection and event-level personalization for importance-based resource distribution, which address inefficient resource allocation. These codesign innovations significantly improve the MFU from 17\% to 37\% on NVIDIA B200 GPUs\footnote{\url{https://www.nvidia.com/en-us/data-center/b200/}}, and yield 2X improvement in scaling efficiency over state-of-the-art approaches. \algname\ has been deployed to major Meta Ads models, achieving significant production impacts.


Deriving predictable scaling laws that govern the relationship between model performance and computational investment is crucial for designing and allocating resources in massive-scale recommendation systems. While such laws are established for large language models, they remain challenging for recommendation systems, especially those processing both user history and context features. We identify poor \emph{scaling efficiency} as the main barrier to predictable power-law scaling, stemming from inefficient modules with low Model FLOPs Utilization (MFU) and suboptimal resource allocation. We introduce \algname, a scalable architecture that systematically improves model efficiency and resource allocation. Our low-level optimizations include Generalized Dot-Product Attention (GDPA), Hierarchical Seed Pooling (HSP), and Sliding Window Attention. Our high-level innovations feature Computation Skip (CompSkip) and Event-level Personalization. These advances increase MFU from 17\% to 37\% on NVIDIA B200 GPUs and double scaling efficiency over state-of-the-art methods. \algname\ is now deployed in major Meta Ads models, delivering significant production impact.
\end{abstract}

